Accelerator-as-a-Service in Public Clouds: An Intra-Host Traffic Management View for Performance Isolation in the Wild

I/O devices in public clouds have integrated increasing numbers of hardware accelerators, e.g., AWS Nitro, Azure FPGA and Nvidia BlueField. However, such specialized compute (1) is not explicitly accessible to cloud users with performance guarantee, (2) cannot be leveraged simultaneously by both providers and users, unlike general-purpose compute (e.g., CPUs). Through ten observations, we present that the fundamental difficulty of democratizing accelerators is insufficient performance isolation support. The key obstacles to enforcing accelerator isolation are (1) too many unknown traffic patterns in public clouds and (2) too many possible contention sources in the datapath. In this work, instead of scheduling such complex traffic on-the-fly and augmenting isolation support on each system component, we propose to model traffic as network flows and proactively re-shape the traffic to avoid unpredictable contention. We discuss the implications of our findings on the design of future I/O management stacks and device interfaces.

==> design-options.tex <==
\section{Design Options}

NIC side solution

\subsection{Host Network Rate Limiting}

Two potential solutions: 
(1) Real system solution: use OVS hardware to rate limit the ports
(2) Re-architect the NIC with more rate limiters

Other solutions: 
\subsection{Multi-tenant DMA}
with IOMMU support

\subsection{Multi-tenant PCIe}

\subsection{Multi-tenant IOMMU}

Host side solution
\subsection{QP mapping virtualization}

\subsection{Profiling based NIC bandwidth allocation}


\section{Desgin: Accelerator Traffic Shaping}

\section{Accelerator Traffic Shaping}\label{sec:design}

\jz{There should be something to cut in this section....}


\begin{figure}
  \centering
  \includegraphics[width=0.99\columnwidth]{./figures/system.pdf}
  \caption{Proposed system with the accelerator management stack. \jz{Limitation: of this system: how could hardware QPs coordinate so that all I/O contention problems can be addressed in this way? Maybe this figure doesn't show this meaning. Ideally, we will have a hardware interface working on not only accelerator devices but also working for coordinating accelerator and NIC and NVMe QPs together. } 
     \label{fig:system}
\end{figure}

\textbf{Should we support separate accelerator QPs?} 
Existing work leverages I/O accelerators by coupling their invocations with the NIC's QPs~\cite{eran2019nica,eran2022flexdriver,lin2020panic,dpdk-compression-accelerator,dpdk-qat-compression}. 
Reusing NIC QPs means that accelerators are hidden from the control plane and dataplane applications. 
In this way, the accelerator can be tightly coupled to 
a particular network I/O path.  
This is feasible to incorporate accelerators in inline mode into network applications without software modifications (e.g., drivers). 
However, once the accelerator is allocated, there is no way to flexibly monitor its utilization, increase its compute capacity, release its cycles, or reallocate it to other requesters. 
% rigidly

We propose to provide a separate set of accelerator QPs from the host perspective. 
Fig.~\ref{fig:system} shows a system overview that has an accelerator interface in hardware and separate accelerator driver in the OS. 
Thus, the OS takes charge of the accelerator resource management with a separate management stack. 
The stack is in parallel with the NIC and NVMe SSD management stacks, rather than be coupled within them. 
With accelerator QPs, I/O accelerators have a management interface that brings information through descriptors, 
such as initialization, configuration, (re)allocation, monitoring and traffic shaping commands from the accelerator manager to the accelerator interface.
Therefore, the manageability for each accelerator I/O flow is improved. For example, the provider can control how many QPs are allocated to each flow for performance benefits or contention management (as observed in Sec.~\ref{sec:understanding}).  
%We also articulate that this system design offers a traffic shaping abstraction for us to manage accelerator resources. 




\textbf{Where should the accelerator traffic shaping functionality exist?}
\kl{You may want to specify what exactly these locations mean}
There are several options for the location of the traffic shaping: hypervisor, user domain (in VMs or containers), or the accelerator interface. We choose to implement traffic shaping at the accelerator interface for two reasons.

First, hypervisors do not always have the permission to know detailed traffic information such as message sizes. 
Additionally, due to host resource contention, high accuracy traffic shaping is sometimes challenging when the hypervisors run in host software.\footnote{For example, to rate limit 100Gbps stably, the software needs to pace 1KB accelerator I/O message every $\sim$80ns on average. Even high-resolution timers in today's software cannot always guarantee such accuracy. } 
Worse, even though in some cases the inaccuracy is acceptable, in-hypervisor traffic shaping still loses its manageability in some systems where hypervisors are bypassed~\cite{sr-iov,kwon2020fvm,azuresmartnic}. 

Second, users themselves can have detailed knowledge to shape their traffic patterns, but they may not know the accelerator's characteristics hosted by the provider. 
In addition, providers cannot rely on users to shape themselves because users are untrusted in the public cloud. 

Our work exploits traffic shaping in the accelerator interface.  
This design option stands out due to the following reasons. 
First, the accelerator interface has local accessibility to the accelerators. 
Thus, it has the traffic observability to accelerators' status, such as queuing effects and ingress/egress bandwidth requirements. 
Second, the interface sits in the middle of the diverse accelerator I/O paths, providing good interposition. 
Thus, it can either work as a switch to forward accelerator traffic in a certain pattern, or  perform on-path processing such as metadata interpretation, scatter-gather, address translation, host network traffic management, and telemetry with hardware counters.  
Third, the interface is customizable by providers, e.g., the descriptors for host-accelerator protocol. %One of the successful feature customized on the device is Azure network virtualization~\cite{azuresmartnic}. 
Forth, the interface is designed in hardware, which naturally delivers high-accuracy traffic management compared with software traffic shaping units. %~\cite{radhakrishnan2014senic}. 



\begin{figure}
  \centering
  \includegraphics[width=0.99\columnwidth]{./figures/protocol.pdf}
  \caption{Proposed traffic shaping protocol. %\jz{Add another line for inline mode between Acc IF and NIC IF?}
  } 
  \label{fig:protocol}
\end{figure}


\textbf{How to perform accelerator traffic shaping (supporting two modes simultaneously)? } 
The host-accelerator traffic shaping is needed in either function call mode or inline mode (e.g., in Fig.~\ref{fig:background}(a) or Fig.~\ref{fig:background}(b)). 
The host-accelerator shaping is performed as follows: 

%To protect each I/O path from being interfered by accelerator traffic, we slightly change the traditional ring buffer protocol. % where tenants \textit{push} notifications to the doorbell registers in the hardware QPs.  
%We enable the accelerator interface to \textit{proactively pull} accelerator-related descriptors and data \textit{on-demand} via DMA. 
%In essence, our approach moves the accelerator traffic initiator from untrusted tenants to infrastructure-managed on-device accelerator interface.  
%%%%% What is the pull-based protocol design %%%%%
Fig.~\ref{fig:protocol} demonstrates our pull-based ring buffer protocol between the host and the accelerator interface (purple path for Tenant A). 
\mycircle{1} To maintain the host-side interface unmodified, we still allow a tenant to push their accelerator I/O requests to the SQ and ring the doorbell register, the same as the vanilla ring buffer protocol from a tenant's perspective. Nevertheless, our interface \textit{ignores} and lazily reacts to such notifications. 
\mycircle{2} The interface fetches the descriptors prepared by the accelerator driver in a pull-based manner. The pulling is a DMA read from the interface to the host memory. %, conducted via SmartNIC-side DMA engines.  
The interface traffic shapes each pulling stream for each tenant. 
The interface processes the descriptors. 
\mycircle{3} The interface fetches DMA data for accelerator computation. %and interprets the metadata inside the descriptor (including I/O message size, accelerated type, a flag bit, and a pointer to the DMA buffer). 
%% omitted info:
% 1) the pointer is an IO virtual address or guest physical address. There still needs IOMMU to translate the address to be host physical address. 
% 2) To process the descriptor efficiently, we use hardware-based interface, with the descriptor format created by the library and processed in hardware. 
\mycircle{4} After the accelerator finishes, the interface DMA-writes the completion message to the CQ in host memory. 

The traffic shaping between the accelerator interface and other interfaces (e.g., NIC QPs or NVMe QPs) is also required in I/O paths existed in either function call mode or inline mode (e.g., in Fig.~\ref{fig:background}(b) or Fig.~\ref{fig:background}(c)). 
This traffic shaping is performed as follows: 


Fig.~\ref{fig:protocol} depicts the traffic shaping for Fig.~\ref{fig:background}(b) case (Green path for Tenant B). 
\mycircle{a} Pull DMA buffer in the host memory under traffic shaper B, the same as \mycircle{1}\mycircle{2} described above. 
\mycircle{b} Dispatch the results of accelerator outputs to the NIC QPs through a protocol converter. 
The converter understands both network transport in use and the accelerator's descriptors in our interface. Since the ingress traffic is shaped, there is no risks of overloading the NIC interface or over-subscribing accelerator bandwidth for Tenant B. 

%%% writing reminders %%%%
%\begin{itemize}
    %\item inline mode that involves accelerator-host communication also supported by this protocol (Fig1(b)). 
    %\item the alternative, where we pair a hardware-based rate limiter with each accelerator VF on the SmartNIC. 
    %\item \jz{Mention the following functionalities in the interface}. DMA message generation, arbitration and split (including address translation).
    %\item Explain how Fig1(c) works in Fig.9. 
%\end{itemize}





\textbf{What traffic metrics to shape?}
The traffic shaping unit for each tenant manages the following parameters: message sizes, burst size of messages, the number of QPs to send/receive, the minimum rate\footnote{The rate of an accelerator traffic stream can be Gbps or IOPS. } (i.e., the SLA), the maximum rate (i.e., how much maximal performance provisioned). 
Note that because of the non-linearity characteristics of accelerators (Sec.~\ref{characterization:accelerators}), the traffic shaping parameters should be re-calculated case-by-case in order to match users' requirements. 
For example, for Tenant A the $X$ Gbps requirement at user level should need $X'$ Gbps ingress traffic at a given traffic pattern (e.g., message size=$M$), accelerator interface resource allocation (e.g., QP number=$Q$), and system setting (e.g.,  PCIe MTU size=$P$), for a given accelerator $A$. 








\textbf{How to determine what traffic pattern to shape?}
If another tenant's traffic is predicted to significantly degrade the throughput of Tenant A, either tenant's traffic patterns should be re-shaped to make the contention predictable while not violating each tenant's SLA. 
The accelerator interface can be configured to re-shape each flow in terms of the metrics we mentioned above. 

%Configure the dataplane 
%DMA message generation, arbitration and split (including address translation). 

%\textbf{Scalalble to hypertenants?}
%the alternative, where we pair a hardware-based rate limiter with each accelerator VF on the SmartNIC.
%per-tenant QPs is shown in Fig.~\ref{fig:protocol}




%The next three questions is for multiple support tenant traffic shaping

%\myparagraph{Full interposition across all QPs}
%With more accelerator types. We will need a driver to manage multiple QPs, talk to them.
%The short term goal for implementation friendly, we can reuse NIC driver. We implement a standalone interface. 

%\myparagraph{How the interface allocate bandwidth across QPs}
%Policy: if not oversubcription, depend on the , if oversubscription .






==> intro.tex <==
\section{Introduction}

Describe two scenarios:
\begin{itemize}
    \item Virtual RDMA network as a service. Bandwidth-oriented and cost driven. 
    \item Virtual NIC accelerator as a service. Bandwidth-oriented and cost driven. 
    \item Virtual local SSD bandwidth as a service. Bandwidth-oriented and cost driven. (FPGA driven local SSDs)
\end{itemize}







==> motivation.tex <==
\section{Understanding Host Network Multi-tenancy Characteristics}

==> open-problems.tex <==
\section{Open Problems}





\section{Open Problems}\label{sec:open}

\jz{Traffic shaping algorithms is a open problem; not 2 to 1, but how to combine. }

\jz{This problem also exist in other I/O system which has not been discussed. }
\jz{Accelerator I/O and other I/O types contention can also be exploited and solved by our proposal. }

\myparagraph{Profile based system management (capacity planning and admission control) vs. adaptive traffic management on the fly}
Some works use pure profiling or learned based system to guarantee isolation. 
This is sometime hard. 

CXL io is PCIe 
CXL complicates the problem but not alternating our findings. 

\myparagraph{CXL device} Traffic shaping is also important for multi-tenancy accelerator services when devices are on CXL fabric. 

\myparagraph{Accelerator chaining} \jz{Local}
Various aspects of the server’s traffic need to chain different types of virtual services together~\cite{de2011application,katsikas2018metron,zhang2018gnet}.
Fig.~\ref{fig:background}(e) illustrates a 4-stage chain for network-attached SSDs. 
SmartNICs enable this virtual service chaining not only because they are already equipped with decryption and compression accelerators, but also because they enable virtual NIC/SSD interface emulation~\cite{li2020leapio,kwon2020fvm,azuresmartnic,}. 
Integrating accelerators into an end-to-end scenario requires us to reconsider all interfaces not only between VM and \verb|vAcc|, but also between \verb|vAcc| and other virtual services. 

\myparagraph{Accelerator disaggregation}
\jz{remote ; open; long term vision. }
Since we leverage accelerators on SmartNICs, efficient network accesses for accelerators are possible. 
Accelerators can connect to the network through end-host networking~\cite{choi2018accelerating,silberstein2016gpunet}, FPGA networking~\cite{sidler2020strom,zilberman2014netfpga,sidler2016low,ruiz2019limago},
or via integrating physical NIC into accelerators~\cite{caulfield2016ltl,eskandari2019modular,korolija2020fpgaabstractions,forencich2020corundum}. 
%Some works even allow accelerators to directly access commodity NIC hardware~\cite{eran2022flexdriver,tork2020lynx,azuresmartnic}. 
Therefore, \design{} has the potential to enhance virtualizable datacenter offloads not only for physical machines local to a certain SmartNIC, but offload-ready to remote VMs as well. 



\myparagraph{Accelerator scalability}
What if each accelerator is not a unit but a spatial array (something like PE arrays of ML accelerator). What if the accelerator array has a specific dataflow type.
\jz{Some inference GPUs can also adopt our technique (when compute is the bottleneck rather than PCIe) (when time multiplexing). }

\myparagraph{When spatialize the accelerator array}
Discrete accelerators and storage accelerators. GPU accelerators and other spatial accelerators. 
AI accelerators
\jz{Chaining}


\myparagraph{Security accelerator sharing}
May leak side channels?
We should distinguish different accelerator types for further


RISC-V cores as accelerators

\myparagraph{Confidential computing needs crypto accelerators very often}

\myparagraph{On-chip accelerators}
now they are treated as PCIe device going through root complex. Still need IOAT DMA on the Intel CPU. The traffic shaping of DMAs is still important for those accelerators. 

IBM data compression: %https://research.ibm.com/publications/data-compression-accelerator-on-ibm-power9-and-z15-processors-industrial-product
IBM encryption: %https://www.ibm.com/downloads/cas/AM1PYZBB

While alternative accelerator placements, like on-chip accelerators~\cite{sapphirerapids-accelerator-profiling,nassif2022sapphirerapids,karandikar2023cdpu,drucker2019vaes,intel-aes-ni,amd-aes} or discrete accelerator cards~\cite{intel-quickassist,kwon2021flexcsv} may offer solutions for delivering accelerator services, SmartNIC accelerators hold a unique position in \textit{proximity to the network interface}. 
For instance, the bump-in-the-wire SmartNIC architecture, which this paper focuses on, allows network data to directly flow through the FPGA from external Ethernet connections~\cite{caulfield2016ltl}, eliminating overheads such as PCIe transactions and host involvement. 
%Some proposals also offload the network stack from the host to SmartNICs~\cite{shashidhara2022flextoe,boo2023f4t,arashloo2020enabling}.
Overall, such direct network accessability gives the potential of tighter \textit{accelerator-network integration}. 
Efficient network accessibility is essential for accelerator disaggregation. 

\myparagraph{RPC abstraction for better usability}


%% Writing reminder: related work
%\input{related-work}

\myparagraph{The role of the FPGA}
Although prototyped on FPGA-based SmartNICs,  layer does not rely on FPGA-specific features. Meanwhile, FPGA-specific benefits~\cite{brant2012zuma,zha2020virtualizingfpga,landgraf2021SYNERGY} such as partial configurations and overlays are orthogonal to \design{}'s benefits. They can enable virtualizable offload models with more features. % such as workload migration and multi-tenancy. 
For instance, accelerators can be reinstalled~\cite{khawaja2018amorphos,byma2014fpgas} or customized by users~\cite{eran2019nica,aws-f1} if they want to buy not only a VM but also a portion of FPGA logic for their own accelerators. 

\myparagraph{Interface implementation: software vs.~hardware}
%Our software-hardware interfaces build upon standard MMIO registers, which could. 
Although we prototype on an FPGA, 
%prototype to implement RTL-level \design{} interface design, to achieve our design goals,
there are no specific restrictions to implement SmartNIC's SoC cores. % to realize near-native SSD performance for LM jobs. 
We use an RTL-level implementation because an SoC-based accelerator hypervisor still triggers non-trivial software overhead. 
Accelerator I/Os still require dozens of usually wimpy SoC cores~\cite{kwon2020fvm,min2021gimbal,li2020leapio}, 
%that usually are wimpy ARM/MIPS cores~\cite{min2021gimbal,li2020leapio}, 
while hardware scales virtualization throughput to hundreds of Gbps with reasonable cost.  
%Second, LM can still cause resource contention and imprecise QoS, whereas the SoC typically has smaller and slower caches/memory against the host~\cite{liu2019ipipe}. 
s on-SmartNIC interface design can also be implemented as an ASIC  with higher clock rates and lower hardware cost for both the  layer and accelerators themselves.



==> related-work.tex <==

Difference between our work and HotNets22~\cite{agarwal2022understandinghostinterconnect}: they focus on congestion in a single-tenant NIC (most study was on RX path). We focus on contention in a multi-tenant I/O accelerator (computation rather than network transmission, more diverse data paths, we care about QPs and message size mixtures). They take more look at the host CPU resources (especially memory), while we exclude memory effects and look more at the NIC interface insiders. (We also did experiments on inter-machine tests and intra-machine single-NUMA node test, we may or may not mention them). 

Some overlaps between our work and HotNets22~\cite{agarwal2022understandinghostinterconnect} if we consider a real cloud scenario: We also have some overlaps. For example, in multi-tenant case, we suffer from host network congestion as well for I/O accelerator traffic; when you take shared memory interconnect contention and CPU contention into account, the contention will be more. 

We did not enable IOMMU in our experiments to study another dimension of host network contention issues when traffic patterns are mixed. 
It is interesting to study our characterizations when IOMMU is on. These are the future works. 

This work~\cite{wang2020fpgacloud} investigated the PCIe overhead of accessing FPGAs in cloud environments for different driver implementations~\cite{wang2020fpgacloud}. 
This work~\cite{tian2021cloudfpga-pcie-contention}, they used PCIe contention to reverse-engineer cloud FPGA infrastructures. 
They instead more extensively study PCIe contention effects due to simultaneous DMA over \textbf{multiple FPGA devices} at once, and use our results for architectural insights into the AWS server infrastructure. 
I found ~\cite{tian2021cloudfpga-pcie-contention} didn't focus on varying traffic patterns like message sizes (Their Fig.12 is a trivial evaluation with only total transfer size at 16KB, 256KB, and 4096KB, not detailed enough). 
They also didn't report contention degress (e.g., how much bandwidth each tenant delivers), but only reporting if contention happens or not. 
On the other hand, our work fits both intra-device induced contention (higher sharing degree) or multi-device contention. 

The good part of ~\cite{tian2021cloudfpga-pcie-contention} is that they study many tenants at once. 
For example, they found there will be 60-80\% probability that a tenant will find a co-located FPGA tenant if more than two tenants exist. 
The other good part of ~\cite{tian2021cloudfpga-pcie-contention}
is that they use PUF to find that there is overlap between instance types of AWS FPGA. In other words, two instances might be mapped to the same physical FPGA hardware. This motivates us to have better capacity planning and admission control algorithms. 

This work\cite{ristenpart2009hey}: Since the initial public deployments of cloud computing
infrastructures, researchers have looked at ways to attack
(and improve) their security. In early Amazon EC2 cloud
architectures involving only CPUs, researchers quickly showed
how to reverse-engineer the infrastructure and place an attacker
VM on the same server as the victim VM. 
The main
method for doing so was through internal IP addresses and
network latencies, which exposed sufficient information about
the underlying setup for effectively 0\% false positives, and a
40\% chance of VM co-location on the same server and CPU
in the AWS EC2 cloud


\jz{The difference and relationship between our work on contention study and multi-device congestion study. Single device congestion study between the host and the Ethernet or RDMA network infrastructure~\cite{agarwal2023hostcc,liu2023hostping}, multi-device congestion study~\cite{li2019prioritygpu,}}
\jz{TODO:  check citations in \cite{tian2021cloudfpga-pcie-contention}}

\jz{This paper~\cite{wang2020fpgacloud} studies the driver efficiency's impact and can be taken care of when we designing our accelerator drivers (also study from NIC drivers~\cite{dpdk-poll-mode-driver} and NVMe drivers~\cite{yang2018spdknvme}.  }

For multi-GPU PCIe network congestions: PCIe congestion has in the past primarily been studied for multi-GPU systems, with PCIe switches becoming a bottleneck when handling traffic from multiple GPUs [7], [9], [11], [34], [36], in part due to a Round-Robin scheduling policy that can lead to severe stalls [21].


%% Related work on accelerator QPs
\cite{kwon2021flexcsv,ruan2019insider,intel-quickassist} those are with separate accelerator QPs. 
They use MMIO as the interface (direct register write)

==> tables/provider-accelerators.tex <==

\begin{table}
    \centering
    \small
    \caption{Examples of accelerators from providers.  \jz{in progress}
    }
    %\vspace{-1em}
    \begin{tabular}{ccc} 
    \toprule
    \textbf{Instance} & \textbf{Type} & \textbf{Description} \\
    \midrule
    AWS AQUA (\verb|ra3.4xl| and \verb|ra3.16xl|) & User (SaaS, no way to specify users) &  FPGAs, provider customized for query acceleration (scans, aggregates, filters)  \\
    %https://aws.amazon.com/blogs/aws/new-aqua-advanced-query-accelerator-for-amazon-redshift/
    AWS Nitro & Provider &  ASIC cards (provider customized)  \\
    Azure NP family & User-defined &  FPGAs (user customized)  \\  %https://learn.microsoft.com/en-us/azure/virtual-machines/np-series
    AWS F1 & User-defined &  FPGAs (user customized)  \\  %https://learn.microsoft.com/en-us/azure/virtual-machines/np-series
    IBM Power9 on-chip accelerators \\
    Oracle \\
    Alibaba FPGA? \\
    
    \bottomrule
    \end{tabular}
\label{table:providers}
\end{table}
    

==> tables/smartnic-acceleration-opportunity.tex <==

\begin{table}
    \centering
    \small
    \caption{Acceleration chances on I/O accelerators.}
    \begin{tabular}{ccc} 
    \toprule
    \begin{tabular}[c]{@{}c@{}}\textbf{Some Tasks at}\\\textbf{Google~\cite{karandikar2021grpcacceleration,karandikar2023cdpu}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{CPU }\\\textbf{Usage}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Acceleration }\\\textbf{Opportunity}\end{tabular} \\

    %\textbf{Acceleration Opportunity}           \\ 
    \midrule
    %\hline
    \textbf{(De)compression}                                                         & 2.9\%                                                                      &  (De)compressor~\cite{dpu-3}                                        \\ 
    %\hline
    \textbf{(De)serialization}                                                                 & 3.45\%                                                                       &     NIC Scatter-gather~\cite{raghavan2021breakfast}                                     \\ 
    \midrule
    \midrule
    \begin{tabular}[c]{@{}c@{}}\textbf{Some Tasks at}\\\textbf{Meta~\cite{sriraman2020accelerometer}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{CPU }\\\textbf{Usage}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Acceleration }\\\textbf{Opportunity}\end{tabular} \\
    
    %\textbf{Acceleration Opportunity}           \\ 
    \midrule
    %\hline
    \textbf{(De)compression}                                                         & 3-15\%                                                                      & ZIP~\cite{bluefield}                                         \\ 
    %\hline
    \textbf{Hashing}                                                                 & 1-4\%                                                                       & SHA~\cite{dpu-3}                                        \\ 
    %\hline
    \textbf{I/O Send/Recv.}                                                          & 4-52\%                                                                      & Special logic                          \\ 
    %\hline
    \textbf{(De)serialization}                                                       & 4-13\%                                                                      & Serializer~\cite{wolnikowski2021zerializer}                                  \\ 
    %\hline
    \textbf{Encryption}                                                              & 1-6\%                                                                       & AES-256~\cite{dpu-3}                                     \\ 
    %\hline
    \textbf{Ranking}                                                                 & 33-58\%                                                                     & 3DES/NN~\cite{liquidio,dpu-3}                      \\ 
    \midrule
    \midrule
    \textbf{Other Tasks}                                                             & \textbf{\textbf{CPU Usage}}                                                 & \textbf{\textbf{Acc. Opportunity}}  \\ 
    \midrule
    %\hline
    \textbf{IP Security~\cite{son2017protego}
    %~\cite{liu2019e3}
    }                                                             & 8 cores (10Gbps)                                                         & IPSec (32Gbps)%~\cite{dpu-3}                               
    \\ 
    %\hline
    \textbf{Data Copy~\cite{kwon2020fvm}}                                                           & 2 cores (18Gbps)                                                         & Special logic (18Gbps)                   \\
    \textbf{Homomorphic Encryption~\cite{heaws,eaws,craterlake}}                                                           &                                                        &                   \\
    \bottomrule
    %\textbf{Deduplication~\cite{pismenny2021autonomous}}                                                           & 2 cores (18Gbps)                                                         & Special logic (18Gbps)                   \\
    %\hline
    \end{tabular}
    \label{table:smartnic-acceleration-opportunities}
\end{table}
    
